Scout: An Experienced Guide to Find the Best Cloud Configuration

Finding the right cloud configuration for workloads is an essential step to ensure good performance and contain running costs. A poor choice of cloud configuration decreases application performance and increases running cost significantly. While Bayesian Optimization is effective and applicable to any workloads, it is fragile because performance and workload are hard to model (to predict). In this paper, we propose a novel method, SCOUT. The central insight of SCOUT is that using prior measurements, even those for different workloads, improves search performance and reduces search cost. At its core, SCOUT extracts search hints (inference of resource requirements) from low-level performance metrics. Such hints enable SCOUT to navigate through the search space more efficiently---only spotlight region will be searched. We evaluate SCOUT with 107 workloads on Apache Hadoop and Spark. The experimental results demonstrate that our approach finds better cloud configurations with a lower search cost than state of the art methods. Based on this work, we conclude that (i) low-level performance information is necessary for finding the right cloud configuration in an effective, efficient and reliable way, and (ii) a search method can be guided by historical data, thereby reducing cost and improving performance.

==> Makefile <==
NAME=paper

TEX = abstract.tex approach.tex conclusion.tex evaluation.tex introduction.tex paper.tex relatedwork.tex

PDF = $(PACKAGE).pdf

all:  $(NAME).pdf

paper.pdf: paper.tex usenix.sty $(TEX)
	pdflatex $<
	- bibtex $(NAME)
	pdflatex $<
	pdflatex $<

usenix.pdf: usenix.tex usenix.sty $(TEX)
	pdflatex $<
	- bibtex -min-crossrefs=999 $(NAME)
	pdflatex $<
	- bibtex -min-crossrefs=999 $(NAME)
	pdflatex $<

clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf $(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE) 

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> acknowledgments.tex <==
\section{Acknowledgments}
\label{sec:acknowledgments}


A polite author always includes acknowledgments.  Thank everyone,
especially those who funded the work. 

==> algorithms/search.tex <==
\begin{algorithm}[htbp]
{
 \SetAlgoLined
 \DontPrintSemicolon
 \DontPrintSemicolon
 %\KwIn{$f$, $\mathit{VM}$, $S$, $M$}
 %\KwOut{The selected deployment configuration}
 $W$ := the workload provided by a user\;
 $S_{i}$ := An initial deployment\;

 \While{does not meet stopping criteria}{
   $S_j, P_j^{pred}$ := select the best from the better choices\;
   $P_j, L_j$ := measure $W$ on $S_j$ and collect low-level metrics\;
   $d$ := performance delta between the actual and predicted values, $\frac{(P_j - P_j^{pred})}{P_j^{pred}}$\;
   adjust\_predictions($S_i$, $d$)\;
   update\_routing\_table($S_j$, $P_j$)\;
   $S_i$ := $S_j$\;
 }
 \caption{Guided Search}
 \label{alg:search}
 }
\end{algorithm}

==> approach2.tex <==
\section{System Design}
\label{sec:approach}


\subsection{Architecture}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/routing_table.pdf}
    \caption{Probabilistic routing table}
    \label{fig:routing_table}
\end{figure}

% high level design
Our approach is search-based method that leverage machine learning model
to eliminate unnecessary exploration steps.

% intuition
Exploration does not converge fast enough because
it requires sufficient data points to conclude.
BOAT is structured Bayesian Optimization designed to
exploit application structure for informed search.
However, in our case, it may still require
significant steps before finding the optimal configuration.
Instead, we combine an offline model which provides
performance inference that can be used for informed search.

% why not just modeling based.
Model based approach might suffer from large variance because
accurately modeling performance is very difficult
CherryPick said it is difficult
PARIS shows high prediction error.

% expert knowledge
We combine A with the help from B


% explain routing table
Routing table, similar to the one in network router,
is a forward table of choosing the next target.

A routing table is generated from low-level metrics collected from
the runtime information ($M$).



A routing table, $RT$

% algorithm


\subsection{Generating Routing Tables}

% how to generate
Probabilistic routing table is generated from a machine learning model
that is trained offline.
The training process is supervised learning in which
a label, \eg{better or worse}, is assigned to input
training data.
The independent variables include
low-level metrics, $\overrightarrow{M}$,
currently evaluated configuration, $C_i$,
and the next configuration to evaluate, $C_j$.
We use classification because xxx.

% generic or independent?

% how about CDP


\subsection{Walk Strategies}

% how many ways to walk
Given a offline model and a start-point configuration,
a walk is a list of steps for finding the best configuration given 
an objective.

Given a start point, there exists many ways to search
towards the optimal solution.
First, the \emph{greedy} strategy picks the next configuration
with the highest probability of bettering the current one.

% need to decide what to compare (collect data first)


\subsection{Model training}

\subsubsection{Data collection}

% spark-perf
\emph{spark-perf} is a performance testing suite for Spark \cite{sparkperf}.
The testing suite provides a wide-range of applications including
supervised learning such as regression and classification modeling,
unsupervised learning such as K-Means clustering,
and statistical tools such as correlation analysis, and principle component analysis.
Besides, \emph{spark-perf} are configurable with application parameters and data sizes.
We use 22 application from \emph{spark-perf}, and they are tested on Spark 1.5.

\emph{HiBench} is a big data benchmark suite for Apache Hadoop and Spark \cite{hibench}.
It is designed for testing batch processing jobs and streaming workloads.
We pick 6 Hadoop and 10 Spark applications, and they are tested on
Apache Hadoop 2.8 and Spark 2.2 respectively.

% configuration space

% low-level metrics





==> system.tex <==
\section{System Design and Implementation}
\label{sec:system}

This section describe our system design and its implementation
as shown in \myfigure{\ref{fig:system_design}}.
We implement the system in Python with
scikit-learn~\cite{scikit-learn} for machine learning libraries and
Boto 3~\cite{boto3} for Amazon web services.


\begin{figure}[t]
 \includegraphics[width=.4\textwidth]{figures/system_design.pdf}
 \centering
 \caption{System design}
 \label{fig:system_design}
\end{figure}


\subsection{Recommendation Engine}
This is the entry point to use \emph{Scout}.
Users specify the workload (program and input data),
the performance or cost requirements,
the architecture choices and the budget.
The recommendation engine then starts the optimization process including
measurements and data collection.
The engine generates routing policy based on new measurements.


\subsection{Performance Monitoring}
For each measurement, we monitor the execution time and
collect low-level performance information.
We use the \emph{Sysstat} package on Linux for system monitoring.
Since we collect only generic performance metrics, other monitoring tools
should work as well.
We choose a five-second sampling period.
Each sample has 72 metrics from
CPU, memory, cache, disk and network components.
These numbers are then aggregated from various-size
samples (per node) and nodes (per cluster).
We follow the similar process of feature transformation
as described in~\cite{Hsu2016}.


\subsection{Routing Policy Generator}

The routing policies are generated from
a machine learning built performance model.
We run 125 workloads in total from \cite{hibench,sparkperf}
with single-node and multi-node deployment.
Please refer to our previous work
for the full list of workloads
and the choices of VM types in the single-node setting~\cite{Hsu2017}.

Regarding the multi-node setting,
we choose 9 VM types
($\{c4, m4, r4\} \times \{large, xlarge, 2xlarge\}$ and
vary the cluster sizes (from 4 to 48).
This combination produces 69 deployment choices.
\myfigure{\ref{fig:search_space}} shows a partial search space
of the \emph{c4} instance family.
These deployment choices allow us to test different scaling behavior,
scale-up, scale-out and the same core counts but with different number of machines.
Overall, our system is designed to tackle the strong scaling problem.


To derive the probability distribution over prediction classes,
we choose \emph{Random Forests} because of
its stability and compute efficiency~\cite{breiman2001random}.
Other learning methods
such as ExtraTree, Gaussian Process and deep neural network (DNN)
can deliver similar modeling effectiveness.


\subsection{Architecture Explorer}
The architecture explore is the implementation of
the proposed search algorithm in \todo{xx}.
The stopping criteria is based on a budget or expected improvement.
We use expected improvement in later evaluation.
When the optimizer does not find any better deployment
in three consecutive times,
it stops the search process.


\subsection{Cloud Controller}
This controller bridges the explorer and the AWS cloud platform.
The controller is responsible for running the workload
with a specific deployment
upon the request from the architecture explorer.


\subsection{Open Performance Database}
We plan to open source the performance database.
As more performance profiles are collected,
\emph{Scout} is able to recommend deployment
for different applications and systems.
Currently, we have tested \emph{Scout} on Apache Hadoop and Apache Spark.

==> tables/multiple_cost_search_path_bo_hadoop_terasort_bigdata.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
{\scriptsize
\begin{tabular}{@{}p{0.2cm}l@{}}
\toprule
\textbf{Step} & \textbf{VM (\#)} \\ \hline
1 & m4.xlarge (20) \\
2 & r4.large (48) \\
3 & c4.large (16) \\
4 & c4.large (4) \\
5 & c4.large (32) \\
6 & r4.large (32) \\
7 & c4.large (40) \\
8 & c4.large (24) \\
9 & c4.large (48) \\
10 & r4.large (16) \\
11 & c4.xlarge (20) \\
12 & r4.large (24) \\
13 & r4.large (40) \\
14 & m4.large (16) \\ \hline
\end{tabular}
}
%\caption{My caption}
%\label{my-label}


==> tables/multiple_cost_search_path_bo_spark1.5_naive-bayes_huge.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
{\scriptsize
\begin{tabular}{@{}lll@{}}
\toprule
     & \#      & VM         \\ \midrule
1    & 20     & m4.xlarge  \\
2    & 48     & r4.large   \\
3    & 16     & c4.large   \\
4    & 4      & c4.large \\
     &        &            \\
     &        &            \\
     &        &            \\
     &        &            \\
     &        &            \\ \bottomrule
\end{tabular}
}
%\caption{My caption}
%\label{my-label}


==> tables/multiple_cost_search_path_scout_hadoop_terasort_bigdata.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
{\scriptsize
\begin{tabular}{@{}lll@{}}
\toprule
     & \#     & VM         \\ \midrule
1    & 24     & m4.large  \\
2    & 6      & m4.large   \\
3    & 4      & m4.2xlarge   \\
4    & 4      & m4.xlarge \\
5    & 12     & m4.large   \\
6    & 6      & m4.xlarge   \\
7    & 4      & c4.xlare  \\
     &        &            \\
     &        &            \\ \bottomrule
\end{tabular}
}
%\caption{My caption}
%\label{my-label}


==> tables/multiple_cost_search_path_scout_spark1.5_naive-bayes_huge.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
{\scriptsize
\begin{tabular}{@{}lll@{}}
\toprule
     & \#     & VM         \\ \midrule
1    & 24     & m4.large  \\
2    & 24     & r4.xlarge   \\
3    & 10     & m4.2xlarge   \\
4    & 24     & m4.xlarge \\
5    & 10     & r4.2xlarge   \\
6    & 8      & m4.2xlarge   \\
7    & 16     & r4.xlarge   \\
     &        &            \\
     &        &            \\
     &        &            \\ \bottomrule
\end{tabular}
}
%\caption{My caption}
%\label{my-label}


==> tables/multiple_time_search_path_bo_hadoop_pagerank_bigdata.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
{\scriptsize
\begin{tabular}{@{}lll@{}}
\toprule
     & \#      & VM         \\ \midrule
1    & 20     & m4.xlarge  \\
2    & 48     & r4.large   \\
3    & 16     & c4.large   \\
4    & 4      & r4.2xlarge \\
5    & 32     & r4.large   \\
6    & 48     & c4.large   \\
7    & 24     & r4.xlarge  \\
     &        &            \\
     &        &            \\ \bottomrule
\end{tabular}
}
%\caption{My caption}
%\label{my-label}


==> tables/multiple_time_search_path_bo_spark1.5_regression_huge.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
{\scriptsize
\begin{tabular}{@{}lll@{}}
\toprule
     & \#      & VM         \\ \midrule
1    & 20     & m4.xlarge  \\
2    & 48     & r4.large   \\
3    & 16     & c4.large   \\
4    & 4      & r4.2xlarge \\
5    & 24     & m4.xlarge   \\
6    & 24     & r4.large   \\
7    & 24     & c4.xlarge  \\
     &        &            \\
     &        &            \\ \bottomrule
\end{tabular}
}
%\caption{My caption}
%\label{my-label}


==> tables/multiple_time_search_path_scout_hadoop_pagerank_bigdata.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
{\scriptsize
\begin{tabular}{@{}lll@{}}
\toprule
     & \#     & VM         \\ \midrule
1    & 24     & m4.large  \\
2    & 24     & c4.xlarge   \\
3    & 12     & r4.2xlarge   \\
4    & 48     & m4.large \\
5    & 12     & m4.2xlarge   \\
6    & 12     & c4.2xlarge   \\
     &        &            \\
     &        &            \\
     &        &            \\ \bottomrule
\end{tabular}
}
%\caption{My caption}
%\label{my-label}


==> tables/multiple_time_search_path_scout_spark1.5_regression_huge.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
{\scriptsize
\begin{tabular}{@{}lll@{}}
\toprule
     & \#     & VM         \\ \midrule
1    & 24     & m4.large  \\
2    & 20     & r4.xlarge   \\
3    & 12     & r4.2xlarge   \\
     &        &            \\
     &        &            \\
     &        &            \\
     &        &            \\
     &        &            \\
     &        &            \\ \bottomrule
\end{tabular}
}
%\caption{My caption}
%\label{my-label}


==> tables/overall_single_cost.tex <==
\begin{table}[]
\centering
\scriptsize
\begin{tabular}{|l|r|r|r|r|l|}
\hline
method & fair               & good & great & optimal & steps \\ \hline
random-4   & 32\% & 2\%   & 0\%     & 0\%         & 4.0 \\ \hline
random-6   & 73\% & 16\%  & 2\%     & 0\%         & 6.0 \\ \hline
random-8   & 93\% & 48\%  & 9\%     & 0\%         & 8.0 \\ \hline
coordinate & 93\% & 84\%  & 60\%    & 37\%        & 8.0 \\ \hline
bo         & 71\% & 50\%  & 21\%    & 0\%         & 5.7 \\ \hline
bo-0.05    & 77\% & 56\%  & 37\%    & 1\%         & 6.2 \\ \hline
scout      & 94\% & 84\%  & 67\%    & 39\%        & 3.7 \\ \hline
\end{tabular}

\caption{Search performance of optimizing operating cost}
\label{tab:search_single_cost}
\end{table}

==> tables/overall_single_time.tex <==
\begin{table}[]
\centering
\scriptsize
\begin{tabular}{|l|r|r|r|r|l|}
\hline
method & fair               & good & great & optimal & steps \\ \hline
random-4   & 44\% & 9\%   & 1\%     & 0\%         & 4.0 \\ \hline
random-6   & 82\% & 37\%  & 6\%     & 0\%         & 6.0 \\ \hline
random-8   & 93\% & 71\%  & 23\%    & 0\%         & 8.0 \\ \hline
coordinate & 90\% & 79\%  & 63\%    & 36\%        & 8.0 \\ \hline
bo         & 86\% & 64\%  & 25\%    & 1\%         & 4.7 \\ \hline
bo-0.05    & 89\% & 75\%  & 44\%    & 1\%         & 5.0 \\ \hline
scout      & 94\% & 83\%  & 64\%    & 40\%        & 2.9 \\ \hline
\end{tabular}

\caption{Search performance of optimizing execution time}
\label{tab:search_single_time}
\end{table}
